Chimera: A Block-Based Neural Architecture Search Framework for Event-Based Object Detection

Event-based cameras are sensors that simulate the human eye, offering advantages such as high-speed robustness and low power consumption. Established Deep Learning techniques have shown effectiveness in processing event data. Chimera is a Block-Based Neural Architecture Search (NAS) framework specifically designed for Event-Based Object Detection, aiming to create a systematic approach for adapting RGB-domain processing methods to the event domain. The Chimera design space is constructed from various macroblocks, including Attention blocks, Convolutions, State Space Models, and MLP-mixer-based architectures, which provide a valuable trade-off between local and global processing capabilities, as well as varying levels of complexity. The results on the PErson Detection in Robotics (PEDRo) dataset demonstrated performance levels comparable to leading state-of-the-art models, alongside an average parameter reduction of 1.6 times.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/3_methodology.tex <==
\section{Methodology}
\label{sec:method}

Event-based cameras are 2D sensors that detect brightness fluctuations at the pixel level. This phenomenon can be quantitatively represented as follows:

\begin{equation}
\small
    \Delta L(x_{k}, y_{k}, t_{k}) \ge p_{k}C
    \label{eq:brightness_change}
\end{equation}

In this equation, $\Delta L$ represents the logarithmic change in the current of a photoreceptor (brightness) at the pixel coordinates $(x_{k}, y_{k})$ at timestamp $t_{k}$. The term $p_{k} \in \{+1, -1\}$ denotes the polarity of the event, indicating that a brightness change that surpasses the threshold (C) in absolute value triggers a positive or negative event \cite{original_dvs_paper}. Each event is defined by the tuple $e_{k} = (x_{k}, y_{k}, p_{k}, t_{k})$. To facilitate the processing of event data, it is common to convert it into an intermediate format that Deep Learning algorithms can easily handle. 
\par 
Chimera has a modular design consisting of fixed and variable computing blocks, also comprising choices of such event conversion. Overall, its structure is inspired by the architecture of Recurrent YOLOv8 (ReYOLOv8) \cite{reyolov8} and consists of a recurrent backbone module for feature extraction from the input and the multi-scale feature fusion and detection heads adopted from the original YOLOv8 model \cite{yolov8}. The NAS in Chimera focuses on finding the best-performing combination of heterogeneous variable blocks for composing the architecture of a recurrent backbone. 

The framework includes multiple steps:
\begin{compactitem}
\item Creation of a design space and benchmarks;
\item Selection of proxy metrics and evaluation of the candidates from the search space; 
\item Evaluation of the resulting Chimera network on the dataset PEDRo.
\end{compactitem}


% step 1 - design or search space

% step 2 search metrics, search score, search algorithm

% step 3 test benchmarks 

% step 4 baseline models




\subsection{Chimera Network Organization}
%\subsection{Base Topology}

%The search space is comprised of SSM, MLP-mixer, convolutional and transformer blocks. 

  
\par 

%\todo[color=red, inline]{Here you do not have a Base Topology, you have base components or search space dimensions. You can have a subsection describing the fixed blocks.}
% {\textcolor{blue}{The base template of this work is ReYOLOv8} \todo[color=red, inline]{WHAT DO YOU MEAN BY TEMPLATE? WHY REYOLOV8? I THINK THE NEXT STATEMENT IS A SUFFICIENT} \cite{reyolov8}. 
% {\textcolor{blue}{In Chimera, the multi-scale feature fusion and detection heads from YOLOv8 are kept. The NAS is focused only on the recurrent backbone. }
%\todo[color=red, inline]{Is this the C2F? if so, state explicitly} 
% {\textcolor{blue}{The use of detection heads from the YOLO family is well-established for event-based detection }
%\todo[color=red, inline]{Here you can give examples of the ReYolo as an example adopting YOLOV8}

% {\textcolor{blue}{
% from where, besides ReYOLOv8, it can be found the adoption of YOLOv6 \cite{yolov6}, as present in \cite{ergo12}, and YOLOX \cite{yolox}, as adopted by \cite{rvt}, \cite{sast}, \cite{get}, and \cite{event-ssm}.
% Figure \ref{fig:chimera_overall} shows the basic structure of the Chimera's recurrent backbone.}

%\todo[color=red, inline]{You are showing the wrong figure. It is repeated in 1 \& 2, I guess 1 is wrong}.
% {\textcolor{blue}{\sout{The first two layers, Stem and Downsample, are downsampling convolutional layers with kernel 3x3 and output channels adjusted during the search. Then, four Chimera layers are stacked in sequence. Then, the SPPF layer from ReYOLOv8 is stacked after the last layer.}}
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.54]{figurinhas/chimera_overall2.png}
    \caption{Structure of the Chimera Network.}
    \label{fig:chimera_overall}
\end{figure}
Figure \ref{fig:chimera_overall} displays the fundamental architecture of Chimera's recurrent backbone, which consists of seven layers. It begins with a variable Event Encoding block, followed by a 3x3 downsampling convolutional STEM layer. The subsequent four layers are called Chimera layers, each having an identical structure but varying compositions. Each of these four layers comprises three components: downsampling, processing, and a memory cell. The downsampling components resemble the STEM layer, while the memory cell is a fixed structure based on ConvLSTM \cite{convlstm}. The ConvLSTM is modeled after a standard LSTM \cite{gers2000learning}, with the critical distinction that the fully connected layers in the LSTM gates have been replaced by convolutional layers, allowing it to effectively process spatial features, similar to the implementations seen in Recurrent Vision Transformer (RVT) \cite{rvt} and ReYOLOv8 \cite{reyolov8}. The Downsample block diminishes the spatial dimensions before passing the features to the variable processing block, which extracts relevant information from the current features, while the following memory cell performs spatiotemporal modeling between the current and previous feature maps. The processing block can utilize any option available in Chimera's component library, and the choice of block for each Chimera Layer is made independently from the others.


% \begin{figure}[ht!]
%     \centering
%     \includegraphics[scale=0.65]{figurinhas/chimera_structure.eps}
%     \caption{Chimera network.}
%     \label{fig:chimera_overall}
% \end{figure}
% {\color{blue} The Chimera layers are structures consisting of three blocks: processing block, memory cell, and downsampling. The processing block is responsible for extracting information from the current features, while the memory cell performs the spatiotemporal modeling between the current and previous maps. Then, the Downsample block reduces the spatial size before sending the feature to the next layer. The processing block and memory cell adopt the same number of input and output channels, while the Downsample modifies the output channel.}
%\vspace{-8mm}
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[scale=0.25]{figurinhas/chimera_layer3.eps}
%     \caption{Chimera basic layer.}
%     \label{fig:chimera_layer}
% \end{figure}
% \subsection{\sout{Building Blocks}}
% \label{sec:blocks}
%\todo[color=red, inline]{You must clarify building blocks for which components in the network. In other words, you can start by stating the fixed blocks and then detail the variable ones, and why you chose to do so?}
% This work adopts two types of convolutional blocks. The first one has the STEM and Downsampling layers that are all 3x3 convolutions. The second one is the modified version C2f from ReYOLOv8 model \cite{reyolov8}, here also called the Cross-Partial Stage (CSP) bottlenecks. 
% {\color{orange} The processing block and memory cell adopt the same number of input and output channels, while the Downsample modifies the output channel. } 
The final layer of the recurrent backbone is a fixed Spatial Pyramid Pooling Fast (SPPF) \cite{spp} block, stacked to Chimera Layer 4 and is inherited from YOLOv8 \cite{yolov8}. Detection within the Chimera framework is carried out using the multi-scale YOLOv8 detection head, considering the findings reported in \cite{reyolov8} as well as the successful application of other YOLO models within the event-based literature \cite{rvt}, \cite{ergo12}, \cite{event-ssm}.

%Basically, in the original LSTM equation \cite{lstm}, the linear layers are replaced by 1x1 2D Convolutions, enabling it to work over spatial features. 


%In the event-based literature, the adoption of the  showed a, which motivated the inclusion of this block in Chimera's library of blocks.
%It consists of two branches, each projected to $\frac{C}{2}$ through linear layers. Then, one branch passes through a 1D convolution and an SSM layer, the selective scan operation from \cite{mamba_original}. Then, the parallel branch will consist only of the convolution. Those branches guarantee a balance between sequential and spatial information extraction. In the end, the features from each branch will be concatenated and passed to an MLP layer. For a structure with $N$ MambaMixers stacked, half of them will utilize the SSM mixer, while the other half will adopt a simple self-attention\cite{mambavision}. In Chimera, only the SSM mixer branch will be adopted.

%Figure \ref{fig:mamba_mixer} shows the mixer block from MambaVision. It consists of two branches, each projected to $\frac{C}{2}$ through linear layers. Then, one branch passes through a 1D convolution and then through an SSM layer, the selective scan operation from \cite{mamba}. Then, the parallel branch will consist only of the convolution. Those branches guarantee a balance between sequential and spatial information extraction. In the end, the features from each branch will be concatenated and passed to an MLP layer. For a structure with $N$ MambaMixers stacked, half of them will utilize the SSM mixer, while the other half will adopt a simple self-attention\cite{mambavision}.

%\begin{align}
%    {h}'(t) &= \textbf{A}h(t) + \textbf{B}u(t) \\
%    y(t) &= \textbf{C}h(t)
%        \label{eq:simple_statespace}
%\end{align}

%where \textbf{A} \in \( \mathbb{R}^{M \times M} \), \textbf{B} \in \( \mathbb{R}^{1 \times M} \), and \textbf{C} \in \( \mathbb{R}^{1 \times M} \) are learnable parameters. The continuous-time parameters are then converted to discrete-time for efficiency, where the zero-order rule is the most adopted. For a timescale $\Delta$, the corresponding \textbf{\( \bar{A} \)} \in \( \mathbb{R}^{M \times M} \), \textbf{\( \bar{B} \)} \in \( \mathbb{R}^{1 \times M} \), and \textbf{\( \bar{C} \)} \in \( \mathbb{R}^{1 \times M} \) discrete-time parameters are given by 

%\begin{align}
%  \textbf{\( \bar{\textbf{A}} \)} &= \exp{(\Delta \textbf{A})} \\
%    \textbf{\( \bar{\textbf{B}} \)} &= {(\Delta \textbf{A})}^{-1}(\exp{(\Delta \textbf{A})} - \textbf{I}) (\Delta \textbf{B})
%    \\
%     \textbf{\( \bar{\textbf{C}} \)} &= {\textbf{C}}
%        \label{eq:discrete_ssm_params}
%\end{align}

%then the whole system can be represented in the discretized form 

%\begin{align}
%    {h}'(t) &= \textbf{A}h(t) + \textbf{B}u(t) \\
%    y(t) &= \textbf{C}h(t)
%        \label{eq:discrete_ssm}
%\end{align}



%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{figurinhas/mamba_block_structure.PNG}
%    \caption{MambaVision Mixer block structure. \cite{mamba}}
%    \label{fig:mamba_mixer}
%\end{figure}


%Although State Space Models have been studied on the event-based detection domain in the form of memory cells \cite{event-ssm}, to our knowledge, this is the first work to study its combination on the point-of-view of feature extraction.

%\subsubsection{Memory Cells}

%In this work, following the implementations from RVT \cite{rvt} and ReYOLOv8 \cite{reyolov8}, a ConvLSTM \cite{convlstm} will be adopted as the only memory cell. Basically, in the original LSTM equation \cite{lstm}, the linear layers are replaced by 1x1 2D Convolutions, enabling it to work over spatial features.

%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=1.0\linewidth]{figurinhas/convlstm.jpg}
%    \caption{ConvLSTM cell.}
%    \label{fig:convlstm}
%\end{figure}


\subsection{Library of Components}
\label{sec:library}

The library supporting Chimera is comprised of various building blocks and options for data encodings. This section will provide a brief overview of each component. Further details regarding their implementations are available in the Supplementary Material.


\subsubsection{Building Blocks}
\label{sec:building_blocks}


\begin{itemize}{
\item {\textbf{Convolutional Layers.} The well-recognized capability of Convolutional Neural Networks (CNNs) to extract features has significantly transformed a variety of computer vision tasks \cite{krizhevsky2012imagenet}. For example, YOLOv8, which serves as the foundation of the Chimera framework, is composed of backbone, neck, and head blocks made entirely of convolutions, like the downsampling convolutions and the C2f blocks adopted for finer feature extraction \cite{yolov8}. Then, besides the convolutional layers on the YOLOv8 detection heads and in the downsampling and SPPF operations from the backbone, the C2f was selected as one of the possible processing blocks for the Chimera Layers.}

\item {\textbf{Transformers.} Transformers are highly powerful in modeling global context information due to the presence of self-attention operations \cite{attention}. However, this operation has quadratic complexity concerning the input size, which incurs computational burdens. In this context, Multi-axis Vision Transformer (MaxViT) \cite{maxvit} is a variation of self-attention with reduced computational complexity. Moreover, it was already successfully adopted in the event domain \cite{rvt}, which motivated us to include it in Chimera's library.}

\item {\textbf{MLP-Mixers.} Multilayer Perceptron (MLP)-Mixers model both local and global relationships through channel mixing and token mixing \cite{mlpmixer}. Token mixing captures spatial information, while channel mixing focuses on feature information. Particularly, WaveMLP is an MLP-Mixer that treats tokens as waves, incorporating amplitude and phase information and introducing a Phase-Aware Token Mixing module (PATM) \cite{wavemlp}. Due to its flexibility and reported performance, WaveMLP was included in the Chimera library.}

\item {\textbf{State Space Models.}
Grounded in continuous-time linear systems, these models have recently gained prominence for their efficiency in parallel processing. A variety of models adhering to this principle have emerged, mainly differing in their matrix representations. The Mamba block, which is included in the library, has attracted significant attention recently, both in the context of Large Language Models (LLMs) \cite{mamba_original} and in the vision domain \cite{mambavision}.}}
\end{itemize}



% \begin{itemize}
% \item \textbf{C2f:} C2f, or Cross-Stage Partial (CSP2f), is a block utilized in YOLOv8 \cite{yolov8} and ReYOLOv8 \cite{reyolov8} models. It enhances speed and accuracy by finely splitting the gradient. C2f includes convolutional blocks along with a bottleneck, which itself is a sequence of convolutional blocks combined with a shortcut connection. 
% \item \textbf{MaxViT:}
% \item \textbf{WaveMLP:} Multilayer Perceptron (MLP)-Mixers were introduced as an alternative to CNNs and Transformers for various computer vision tasks. They achieve efficient modeling of both local and global relationships through channel mixing and token mixing \cite{mlpmixer}. Token mixing captures spatial information, while channel mixing focuses on feature information. However, a limitation of vision MLPs is their method of aggregating tokens. WaveMLP addresses this challenge by treating tokens as waves, incorporating amplitude and phase information, and introducing a phase-aware token mixing module (PATM) \cite{wavemlp}. Due to its flexibility and reported performance, WaveMLP was included in the Chimera library.
% \item \textbf{Mamba:} Mamba block was evolved from State Space Models (SSMs), a continuous-time linear system efficient in n parallel processing. 
% \end{itemize}



\subsubsection{Data Encodings}
\label{sec:encoding}
% \sout{Alongside the blocks mentioned in Section \label{sec:blocks}, some data encodings were also included in the library.} \todo[color=red, inline]{what library?}

To allow a dense neural architecture to effectively process input events, these events must be converted into a grid-like format \cite{red_megapixel}. Various encoding schemes have been proposed, each varying in its capacity to capture events. In our study, we concentrate on the Volume of Ternary Event Images (VTEI) \cite{reyolov8}, Mixed-Density Event Stacks (MDES) \cite{mdes}, Stacked Histograms (SHIST) \cite{rvt}, and Temporal Active Focus (TAF) \cite{aed-taf} encodings. The VTEI format was chosen for its simplicity, high throughput, efficient compression, and positive results demonstrated in ReYOLOv8 \cite{reyolov8}. MDES shares similarities with VTEI and has shown promising performance in Depth Estimation \cite{mdes}. SHIST is included due to its utilization in multiple studies within the event-based object detection literature \cite{rvt}, \cite{event-ssm}, \cite{sast}. The mentioned formats are based on the accumulation of events across bins, while TAF employs a FIFO-based approach \cite{aed-taf}, thereby enhancing the diversity of the library.
%\todo[color=red, inline]{You can do a proper comparison table and keep the paragraph to illustrate why the encoding can impact performance and should be considered in our work.}


% \subsubsection{Problem Formulation}
% \label{sec:metrics:fitness}

\subsection{Chimera-NAS}
\label{sec:metrics:chimeraNAS}

\subsubsection{Search Metrics}
\label{sec:metrics}


\label{sec:metrics:zen}
%\todo[color=red, inline]{the following are Network evaluation scores perhaps, or search metric, but not performance metric. The performance metrics can be mAP, convergence speed, ...etc. that you use to report the performance of your proposal. Also, at the begning of section 3.4 you should state that there are many scores that are used for Zero-shot NAS, but based on the survey XX you dedicded to use YY because of ZZ}
 
%As it was mentioned in Section \ref{sec:zershotnas} Zero-Shot NAS gives a flexibility of choosing proxies to select the best candidate neural blocks. 
Chimera-NAS is inspired by ZS-NAS, which provides the flexibility to choose proxies for selecting the best candidate neural blocks. In this study, we selected several ZS-NAS proxies from a range of existing options \cite{survey_zsnas}, including gradient-based accuracy proxies such as Zen-Score \cite{zenscore} and the Neural Tangent Kernel (NTK) Condition Number \cite{ntk}, along with naive proxies based on the number of parameters, denoted as \textit{\#Params}, and Multiply-Accumulate (MAC) operations. Additionally, a diversity index was introduced to ensure heterogeneity within the architecture. Together, these components address multiple objectives to achieve a balanced structure.


%there are many scores that are used for Zero-shot NAS, but based on the survey XX you dedicded to use YY because of ZZ, zen-score and Neural Tangent Kernel Condition Number (NTK) , model parameters and complexity.  



%may be Kendall tau should be introduced



\begin{itemize}
\item {\textbf{Zen-Score}}
% \subsubsection{Zen-score}
The expressive capacity of a network refers to its ability to effectively capture complex relationships within the input data. 


For vanilla CNNs, it can be associated with Gaussian complexity according to 
\begin{equation}
\small
    \phi(f) = \log{E_{\mathbf{x}, \mathbf{\theta}} \|\mathbf{  \nabla_{\mathbf{x}}f(\mathbf{x}|\mathbf{\theta})}\|_{F}}
    \label{eq:phi-score}
\end{equation}
where $\mathbf{x}$ is the input, $\mathbf{\theta}$ the network parameters, and $f(.)$ is the network backbone with the last feature before the Global Average Pooling (GAP) operation. The formulation from Equation \ref{eq:phi-score} considers a network without Batch Normalization (BN) layers. However, this leads to problems such as overflow when applied to deep networks. The Zen-score solved this problem by introducing BN layers and considering their variance into the score computation \cite{zenscore}. Furthermore, to avoid adopting the backward propagation from Equation \ref{eq:phi-score}, they calculate the score according to the finite differential
\begin{equation}
\small
    \Delta = {E_{\mathbf{x}, \mathbf{\epsilon}} \|\mathbf{ f(\mathbf{x}) - f(\mathbf{x} + \mathbf{\alpha}\mathbf{\epsilon})}\|_{F}}
    \label{eq:zen-differential}
\end{equation}
where $\epsilon$ is a random disturbance and $\alpha$ is an adjust parameter for this noise. Then, the Zen-score is given by:
\begin{equation}
\small
    Zen(f) = \log(\Delta) + \sum_{i}\log(\sigma_{i})
    \label{eq:zen}
\end{equation}
where $i$ refers to the index of the BN layers, each with its respective standard deviation $\sigma_{i}$. Originally, both $\mathbf{x}$, $\mathbf{\theta}$, and $\mathbf{\epsilon}$ were taken from a standard Gaussian Distribution \cite{zenscore}. Also, in Chimera, $f(.)$ will consider the whole backbone block, including the SPPF block. 
\item{\textbf{Neural Tangent Kernel (NTK) Condition Number}}
% \subsubsection{Neural Tangent Kernel Condition Number}
% \label{sec:metrics:ntk}
The NTK (Neural Tangent Kernel) of a Neural Network can be expressed as follows:

\begin{equation}
\small
    \Theta(x,x') = \mathbf{J}(x)\mathbf{J}(x')^T
    \label{eq:ntk}
\end{equation}
where $\mathbf{J}(x)$ represents the Jacobian evaluated at (x) with respect to the parameters $\theta$. It has been demonstrated that the training dynamics of a neural network under gradient descent can be characterized by the conditioning of its NTK matrix, which is given by:

\begin{equation}
\small
    NTK_{cond} = \frac{\lambda_{0}}{\lambda_{m}}
    \label{eq:ntk_cond}
\end{equation}
where $\lambda_{0}$ and $\lambda_{m}$ denote the lowest and highest eigenvalues of $\Theta(x,x')$, respectively. A well-conditioned NTK matrix is linked to enhanced trainability, and a negative correlation between NTK conditioning and test-set accuracy for image classification tasks has also been reported \cite{ntk}.

\item{\textbf{Model Parameters and Complexity.}}
% \subsubsection{Model Parameters and Complexity}
%\label{sec:metrics:params}
The number of parameters in a model and its complexity, measured in terms MACs, have been found to exhibit a certain degree of correlation with the model's test accuracy. These factors will also be included in the analysis of this work \cite{survey_zsnas}.




%\subsection{Zero-Shot Neural Architecture Search}

%%%%%%%%%%%%%%% here I talk about the basic definition of Zero-Shot NAS
%Proxies are used to avoid undergoing all the training and validation processes \cite{survey_zsnas}
%%%%%%%%%%%%%%%%%% Gradient-Based 

%Gradient norm, the sum of norms of the gradient vector according to each layer \cite{gradnorm}. SNIP, to consider the influence of parameters on the forward pass, takes the absolute value of the sum of the inner products between each layer's parameters and gradients \cite{snip}. At the same time, Synflow uses the same metric but keeps the signs \cite{synflow}. They consider only the first-order derivatives of the NNs. GraSP is a proxy that also considers the second-order derivatives \cite{grasp}. 

%GradSign can measure convergence properties of neural networks by analyzing the parameter-wise uniformity across several training samples \cite{gradsign}.

%It was shown that the Fisher Information is related to the second-order Taylor expansion approximation of a neural network \cite{fisherinformation}.

%Jacobian Covariant is an approach based on analyzing the eigenvalues of a covariance matrix that considers the gradient regarding the input data, besides the ones taken concerning the activations and parameters \cite{jacob_cov1} \cite{jacob_cov2}.

%The Zen-score measures the expressivity of a model by averaging its Gaussian complexity according to random sample inputs and perturbations. Equivalent to the gradient norm with respect to the input instead of the parameters \cite{zenscore}.

%The Neural Tangent Kernel (NTK) Condition Number measures the trainability of a neural network by analyzing whether the NTK matrix, which is associated with the training dynamics of neural networks, is ill-conditioned or not \cite{ntk}.
%%%%

%The number of distinct sections that a network can split its input space can describe the expressivity of a network, being adopted in some works \cite{linearregions}, \cite{jacob_cov2}.

%logdet -> jacov_cov2 

%The NN-Mass was adopted to study the influence of the network topology on the gradient flow \cite{nnmass}, while an extension NN-Degree was proposed by relaxing some width constraints \cite{nndegree}. The spectrum of the Neural Network Gaussian Process (NNGP) was proved to have connections to convergence rates \cite{nngp}.

%%%%

%Other quantities, such as the number of parameters and MACs, have also been evaluated as proxies for the test accuracy of Neural Networks, showing good results in some cases \cite{survey_zsnas}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item{\textbf{Diversity Index.}}
% \subsubsection{Diversity Index}
% \label{sec:metrics:diversity}
To assess the distribution of different types of blocks within a given architecture, we introduce an index to measure architectural diversity. Let $\textbf{B}(f) \in \mathbb{R}^{N \times 1}$ represent a vector where $N$ denotes the number of blocks available in a particular library. Each entry in this vector corresponds to the count of a specific block in the architecture $f$. The Diversity Index $D(f)$ for this architecture can be defined as follows:
\begin{equation}
\small
D(f) = 1 - \frac{\sum_{\forall{(i,j)}, j > i, i \neq j}{|\mathbf{B}(f)_{i} - \mathbf{B}(f)_{j}|}}{S}
    \label{eq:diversity_index}
\end{equation}
where ${\mathbf{B}(f)}_{i}$ represents the entries of the vector $\textbf{B}(f)$, and $S$ is a scale factor related to the maximum value that the summation term can attain. This formulation is designed such that when diversity is at its minimum—indicating that the architecture is homogeneous and consists of a single type of block—$D(f)$ is equal to $0$. Conversely, if there is no repetition in the block choices across all Chimera Layers, $D(f)$ will equal $1$.
\end{itemize}



\subsubsection{Search Space}

The design space $\mathcal{F}$ of Chimera includes a variety of modules and parameters, notably event encoding and processing blocks. The encoding blocks convert the input stream of events into formats such as VTEI, SHIST, MDES, or TAF, which are discussed in detail in Section \ref{sec:encoding}. For this study, the number of temporal bins assigned for the input representation is set to five. Following this, the output channel $Ch$ will be specified at the STEM layer, defined by a 3x3 convolution with a stride of 2.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Chimera Design Space}
\footnotesize
\centering
\label{tab:chimera}
\begin{tabular}{|l|c|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\#}} & \textbf{Layer}                                                                 & \multicolumn{1}{c|}{\textbf{Search focus}}                               & \multicolumn{1}{c|}{\textbf{Choices}}                                            \\ \hline
1                                 & \multicolumn{1}{l|}{Encoding}                                                  & Encoding type                                                           & \begin{tabular}[c]{@{}l@{}}VTEI, SHIST, \\ MDES, TAF\end{tabular}                \\ \hline
2                                 & \multicolumn{1}{l|}{STEM}                                                      & Output Channel $Ch$                                                                & 16, 24, 32, 40, 48                                                               \\ \hline
\multirow{5}{*}{3-6}              & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Chimera \\ Layers 1-4\end{tabular}} & Multiplier $M_i$                                                          & \begin{tabular}[c]{@{}l@{}}1, 1.25, 1.33, 1.50, \\ 1.66, 1.75, 2.00\end{tabular} \\ \cline{3-4} 
                                  &                                                                                & \begin{tabular}[c]{@{}l@{}}Block and \\ Block Params\end{tabular}     & \begin{tabular}[c]{@{}l@{}}C2f, MaxViT, \\ Mamba, \\ WaveMLP\end{tabular}   \\ \cline{3-4} 
                                  &                                                                                & \begin{tabular}[c]{@{}l@{}}Repeats \\ (Except Mamba)\end{tabular}  & 1, 2, 3                                                                          \\ \cline{3-4} 
                                  &                                                                                & \begin{tabular}[c]{@{}l@{}}Heads \\ (Mamba only)\end{tabular}           & 1, 2, 3                                                                          \\ \cline{3-4} 
                                  &                                                                                & \begin{tabular}[c]{@{}l@{}}Head multiplier \\ (Mamba only)\end{tabular} & 1.0, 1.25, 1.5, 2.0                                                              \\ \hline
\end{tabular}
\end{table}

For each Chimera layer, a multiplier $M_{i}$, a processing block, and its corresponding parameters $Block$ and $Block Params$ will be selected. The parameter $Repeats$ is applicable for all blocks, except Mamba. For the C2f, this parameter represents how many bottleneck blocks will be stacked inside its structure, and for the remaining ones, it represents how many of each structure will be stacked together. For Mamba, the number of heads will also be considered a parameter, and a head multiplier will scale the number of heads of a given Mamba block according to its predecessor. Considering all the possible choices, around 20,000 combinations can be generated from this model generator. Table \ref{tab:chimera} summarizes the Design Space for Chimera. More details about the implementation of each block can be find in the Supplementary Material.

%\todo[color=red, inline]{What is ZS-Nas? also, here you should be discussing abstract definitions, because later you drop NTK} 
\subsubsection{Chimera-NAS Algorithm}
\label{ref:chimera-nas}
%\todo[color=red,inline]{Before getting into the full Chimera-NAS algorithm, you need to detail its components, the search space, the search score, and the search algorithm}
% \todo[inline]{ what is Zen-NAS?}
% \sout{The Chimera-NAS algorithm follows an analogous idea to the one adopted for Zen-NAS.} 
The Chimera-NAS Algorithm operates in two stages. In the first stage, it generates and selects architectures using an Evolutionary Algorithm, favored for its simplicity and effectiveness, with prior results in the ZS-NAS domain \cite{zenscore}. The Fitness Score can be calculated based on any of the metrics described in Section \ref{sec:metrics}, or as a combination of these metrics. For a given design space $\mathcal{F}$, the optimization problem that Chimera-NAS seeks to solve to identify an effective architecture can be expressed as follows:

\begin{equation} \label{eq:chimera_optm}
\small
\begin{aligned}
& \underset{f \in \mathcal{F}}{\text{max}}
& & F = \alpha \mathbf{W}\cdot\mathbf{Z}(f) + (1- \alpha)D(f) \\
& \text{s.t.}
& & {Params(f)} \leq \text{$MAX_{\text{Params}}$}.
\end{aligned}
\end{equation}
where $\mathbf{Z}(f)$ $=$ $[Zen(f), MACs(f), NTK_{cond}(f)]$ is a vector that includes the ZS-NAS proxies for the architecture $f$, weighted according to the vector $\mathbf{W} \in \mathbb{R}^{3 \times 1}$; $D(f)$ represents the Diversity Index from Equation \ref{eq:diversity_index}; $Params(f)$ indicates the number of parameters in the architecture $f$; $MAX_{\text{Params}}$ is the upper limit on the number of parameters; and $\mathbf{\alpha} \in [0,1]$ is a constant that regulates the diversity of the architectures. {Kendall's Tau and Spearman's R are used to evaluate correlation between NAS proxies and ground truth. }

In the second stage, the top five architectures identified by the ZS-NAS are trained for 100 epochs. Ultimately, the architecture that achieves the highest mean Average Precision (mAP) is selected. This second step is crucial for reducing the inherent inaccuracies associated with proxy-based methods and fine-tuning the resulting architecture.



\begin{algorithm}
\footnotesize
    \caption{Chimera-NAS Algorithm}
    \begin{algorithmic}[1]
                           \STATE  \textbf{------------------------- First Stage: ZS-NAS  ----------------------------- }
        \STATE \textbf{Input:} Population size $N$, Search space $S$, Number of iterations $I$, Maximum Number of Parameters per architecture $Max_{Params}$, Population $P$, Fitness score $F$
        \STATE \textbf{Initialize:} $P \leftarrow \emptyset$
        
        \FOR{$i = 1$ \textbf{to} $N$}
            \STATE Create individual $I_i$
            \STATE Profile $I_i$ in terms of the ZS-NAS proxies
            \STATE Append $I_i$ to the population $P$
        \ENDFOR

        \FOR{$j = 1$ \textbf{to} $I$}
            \STATE Select a random individual $I_k$ from $P$, where $k = 1, \ldots, N$
            \STATE Apply Mutation to $I_k$, creating the individual $I_{k+1}$
            \IF{$Params(I_k) > Max_{Params}$}
                \STATE \textbf{goto} line 9 
            \ELSE
                \STATE Append $I_{k+1}$ to $P$
                \STATE Calculate the fitness score $F$ for $P$
                \STATE Remove the individual with the lowest $F$ from $P$
            \ENDIF
        \ENDFOR
        \STATE \textbf{\textbf---------------------- Second Stage: Fine-Tuning  ------------------------ }
        \STATE Choose the five individuals $I_k$ with the highest fitness scores and perform training for 100 epochs each
        \STATE \textbf{Output:} The individual $I$ with the highest mAP as the architecture output

    \end{algorithmic}
           \label{alghtm:chimera}

\end{algorithm}


\subsection{Dataset}
\label{sec:datasets}

 The PErson Detection in Robotics (PEDRo) dataset, focusing on robotics applications, is the dataset evaluated in this work. Captured in Italy using a handheld camera, PEDRo includes recordings of individuals in various scenes, lighting conditions, and weather scenarios, with 43k labels. The data was obtained using a DAVIS346 camera with a resolution of 346x260 pixels. To date, PEDRo is the only large-scale, real-world event-based dataset specifically tailored for robotics applications \cite{pedro}. In all instances, the events were aggregated into intermediate representations utilizing constant time windows of 40 ms, as adopted in previous works \cite{pedro}, \cite{reyolov8}. Results for another dataset, the Prophesee's Generation 1 Automotive Dataset (GEN1) \cite{gen1}, are included in the Supplementary Material.
 %The second dataset, Prophesee's Generation 1 Automotive Dataset (GEN1), was recorded in France and encompasses various weather and illumination scenarios incorporating pedestrians and cars \cite{gen1}.

%\begingroup
%\renewcommand{\arraystretch}{1.0}
%\begin{table}[ht!]
%\centering
%\small
%\caption{Dataset adopted in this work.}
%\label{tab:datasets}
%\begin{tabular}{ccccc}
%\hline
%\textbf{Dataset}                                                          & \textbf{Focus} & %\textbf{Classes} & \textbf{Resolution} & \textbf{Labels} \\ \hline
%\begin{tabular}[c]{@{}c@{}}PEDRO\\ \cite{pedro}\end{tabular} & Robotics       & 1                & 346x260             & 43k             \\ \hline
%\end{tabular}
%\end{table}
%\endgroup

\subsection{Chimera Benchmark}
\label{sec:benchmarking}

%A benchmark with some architectures from the Design Space was created to align how well the proxies can predict the test set performance. 
To evaluate the accuracy of the selected proxies in predicting test set performance, a benchmark was created using a subset of architectures from the Design Space. The PEDRo dataset was chosen for this evaluation due to its relatively small size. Each model was trained for 50 epochs, providing an effective compromise between runtime and convergence, and the mAP for the test set was recorded. Additionally, the Zen Score, MACs, number of parameters, and $NTK\_{cond}$ were documented. This analysis involved running 250 randomly generated heterogeneous models. Initially, each model was trained using VTEI, MDES, TAF, and SHIST representations, with 5 temporal bins each. %The metrics analyzed included mAP@0.5:0.95, which served as the ground truth for model comparison, alongside the metrics mentioned in Section \ref{sec:metrics}, which act as proxies for test set performance. 

Two correlation measures assessed how effectively the proxies approximate the mAP ground truth. One of these, Kendall's Tau, compares the ranking of models based on mAP and the proxies. The other metric used is Spearman's correlation, which measures the degree of monotonicity between the two variables, in this case, the proxies and the mAP \cite{survey_zsnas}.

%\subsubsection{Baseline Models}
%\label{sec:benchmarking:baseline}

% {\color{orange}The baseline models are chosen from the literature specifications regarding the blocks presented in Section \ref{}.} 
%{\color{violet} The C2f and MaxVit baselines were previously used in ReYOLOv8n \cite{reyolov8} and  RVT \cite{rvt} for event-based data, and this work adopts their established specifications. For WaveMLP and MambaVision, since no prior studies have explored these blocks in the event-based domain, their specifications were adapted from their ImageNet-1k backbones. Some modifications must be done to fit a Chimera backbone.  }
% \sout{The C2f-baseline follows the same specifications as ReYOLOv8n \cite{reyolov8}, while the MaxViT-baseline follows the specifications from RVT \cite{rvt}. For WaveMLP and MambaVision, as there were no works in the literature studying those blocks on the event-based domain, the specifications were chosen from their ImageNet-1k backbones. Some modifications must be done to adapt them to the template used in this work, as seen in Figure \ref{fig:chimera_overall}.} 
%For example, RVT adopts a single 7x7 convolution with stride 4 as the stem instead of using two 3x3 convolutions with stride 2, as defined in the template of this work. Nonetheless, the original WaveMLP architecture does not use any convolutional layer for downsampling at the token level. To guarantee the compatibility between those architectures and the Chimera's topology, their processing block specification was used to make the Chimera Layers while keeping the downsampling convolutions and Chimera's stem. The configurations are specified on the supplementary materials, and a comparison between this adaptation and their original configurations is presented, showing that they can perform even better through these modifications.

%\subsubsection{Benchmark Evaluation}
%\label{sec:benchmarking:eval}
%\todo[inline]{Kendall's tau was never introduced}


%Firstly, given two ordered sets with the same elements, Kendall's tau is a correlation metric that calculates how much they agree. Kendall rank correlation coefficient. 

%\begin{equation}
%    \tau = 1 - \frac{2 \times [d_{\Delta}(P_{1}, P_{2})]}{N(N-1)}
%    \label{eq:kendall_tau}
%\end{equation}

%where $d_{\Delta}(P_{1}, P_{2})$ is the number of elements not common to the sets of ordered pairs $P_{1}$ and $P_{2}$, and $N$ is the total number of elements on the set. 



\subsection{Training Procedure}
\label{methods:training}


For both the benchmark and final performance analysis, the same set of hyperparameters will be applied to each dataset, consistent with the procedures outlined in ReYOLOv8 \cite{reyolov8}. An image size of 320x256 was utilized for both datasets to enhance compatibility during the search process across different blocks and datasets. The models were trained using Stochastic Gradient Descent (SGD) with weight decay and a linear learning rate schedule. Given the recurrent nature of the architectures \cite{reyolov8}, Truncated Backpropagation Through Time (T-BPTT) \cite{tbptt} was employed. The benchmarks were trained for 50 epochs, while the final architectures were trained for 100 epochs after the searches were completed. All runs involving PEDRo, along with the executions of the Chimera-NAS algorithm, were conducted on a V100 GPU. Additional details can be found in the Supplementary Material.



==> sec/4_results.tex <==
\section{Results}
\label{sec:results}


\subsection{Evaluation of the Chimera Benchmark}
\label{sec:results:bench}


\subsubsection{Analysis of ZS-NAS proxies and event encodings}
\label{sec:proxies_and_encodings}
For the created benchmarks, the relationship between the ZS-NAS proxies and the event encodings was studied via analyzing the correlation between the rankings generated from these scores using Kendall’s correlation and their actual mAP rankings. The results are illustrated in Figure \ref{fig:cor_data_format}a. On average, the Zen Score demonstrated the best performance among other proxies, followed by the number of MACs and the total number of parameters. The NTK exhibited a negative correlation with the actual mAP, not exceeding 0.2 in absolute value. Furthermore, the computation time for NTK was significantly higher than that required for the Zen Score. Consequently, NTK was excluded from further analysis.


% To first assess the relationship between the ZS-NAS proxies and the event encodings in the benchmarked architectures, we analyzed the correlation between their actual mAP rankings and the rankings provided by these scores using Kendall's correlation. The results are displayed in Figure \ref{fig:cor_data_format}. On average, the Zen Score exhibited the highest performance among the proxies, followed by the number of MACs and the total number of parameters. The NTK, as previously reported, showed a negative correlation with the actual mAP; however, this correlation did not exceed 0.2 in absolute value. Furthermore, the computation time for NTK was significantly greater than that for the Zen Score. As a result, it was decided to exclude this proxy from further analysis.


%\todo[color=red, inline]{what relationship between what architectures? Do you mean the relation between the scores and performance?}
%\todo[color=red, inline]{Did you consider only the hetero? if so, why did you neglect the homogeneous?}
%\todo[color=red, inline]{what calculation, and why is hight bad?}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figurinhas/kendall_tau_enc3.eps}
%     \caption{Kendall's Correlation between the different proxies and data formats, for the full heterogeneous architectures.}
%     \label{fig:cor_data_format}
% \end{figure}

\begin{figure}[!t]
\centering
    \begin{subfigure}[]{0.5\textwidth}
        \includegraphics[width=1\textwidth]{figurinhas/kendall_tau_enc3.eps}
        \caption{}
    \end{subfigure}
\hspace{3mm}
    \begin{subfigure}[]{0.33\textwidth}
        \includegraphics[width=1\textwidth]{figurinhas/mAP_box.png}
        %\vspace{3mm}
        \caption{}
    \end{subfigure}
\caption{a) Kendall's Correlation between the different proxies and data formats, for the full heterogeneous architectures.; b) Distribution of the mAPs for the different data encodings analyzed in the benchmark.}
\label{fig:cor_data_format}
%\vspace{-0.1in} 
\end{figure}


Figure \ref{fig:cor_data_format}b presents box plots of the mAP values for all heterogeneous architectures in the benchmark, grouped by encoding format. The results indicate that SHIST, MDES, and VTEI outperform TAF, whereas in the previous analysis, SHIST and TAF demonstrated a better relationship with the proxies than MDES and VTEI. Since SHIST demonstrated a superior performance in both evaluations, it was decided to use it for the subsequent experiments. 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figurinhas/mAP_box_plot.png}
%     \caption{Distribution of the mAPs for the different data encodings analyzed in the benchmark.}
%     \label{fig:map_across_values}
% \end{figure}


Based on the results presented in Figure \ref{fig:cor_data_format}, a decision was made to explore further a fitness function that combines only the Zen Score and the number of MACs proxies. The number of parameters was excluded from the main function and instead treated as a constraint during the search process. {Table \ref{tab:max_correlation} reflects the impact of various weight combinations for the Zen Score and MACs on their corresponding Kendall's and Spearman's correlations relative to the mAP at 50 epochs, derived from the full heterogeneous subset of SHIST in the Chimera benchmark} 
% \sout{Table \ref{tab:max_correlation} displays various combinations of weights for the Zen Score and MACs, along with their corresponding Kendall's and Spearman's correlations concerning the mAP at 50 epochs for the full heterogeneous subset of SHIST in the Chimera benchmarking.} 
The data reveals that the correlations increase up to a point when 60\% of the score is derived from the Zen Score and 40\% from MACs. Beyond this combination, the correlations begin to decline. Consequently, these weights were selected for use in the following experiments.



\begin{table}[]
\centering
\footnotesize
\caption{Kendall's and Spearmans' Correlations for different weighings of Zen Score and MACs for the SHIST subset of the full heterogeneous benchmark.}
\label{tab:max_correlation}
\begin{tabular}{|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Zen\\ Weight\end{tabular} & \begin{tabular}[c]{@{}c@{}}MACs\\ Weight\end{tabular} & \begin{tabular}[c]{@{}c@{}}Kendall's\\ Tau\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spearman's\\ R\end{tabular} \\ \hline
0                                                    & 1.0                                                   & 0.35                                                    & 0.50                                                   \\ \hline
0.1                                                  & 0.9                                                   & 0.39                                                    & 0.55                                                   \\ \hline
0.2                                                  & 0.8                                                   & 0.42                                                    & 0.60                                                   \\ \hline
0.3                                                  & 0.7                                                   & 0.45                                                    & 0.62                                                   \\ \hline
0.4                                                  & 0.6                                                   & 0.47                                                    & 0.65                                                   \\ \hline
0.5                                                  & 0.5                                                   & 0.48                                                    & 0.67                                                   \\ \hline
\textbf{0.6}                                         & \textbf{0.4}                                          & \textbf{0.49}                                           & \textbf{0.67}                                          \\ \hline
0.7                                                  & 0.3                                                   & 0.48                                                    & 0.66                                                   \\ \hline
0.8                                                  & 0.2                                                   & 0.46                                                    & 0.64                                                   \\ \hline
0.9                                                  & 0.1                                                   & 0.44                                                    & 0.62                                                   \\ \hline
1.0                                                  & 0.0                                                   & 0.41                                                    & 0.59                                                   \\ \hline
\end{tabular}
\end{table}




%Figure \ref{fig:benchmark_map_vtei} shows a box plot with the mAPs obtained from training the models with the benchmark specifications for the four homogeneous configurations and the heterogeneous classes. The benchmarks for ReYOLOv8n and MaxViT-Base are also included, adopting VTEI as a data format. It can be seen that the Full-MLPs, C2fs, and Heterogenous models have the best performance, with a considerable amount of cases surpassing the baselines. On the other hand, the MaxViT and Mamba models present an inferior performance, barely outperforming the MaxViT-Base baseline.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figurinhas/MAP.png}
%    \caption{mAP distribution for VTEI.}
%    \label{fig:benchmark_map_vtei}
%\end{figure}

%Figure \ref{fig:benchmark_zenscore_vtei} shows the distributions of the ZenScores for the same models presented before. It can be seen that the ordering of the plots follows the same behavior as the one found on the map in Figure \ref{fig:benchmark_map_vtei}. It is also in consonance with the findings shown in Table \ref{tab:Regression Weights}, which highlights a strong relationship between the ZenScore and the test-set performance of the model.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figurinhas/zenscore.png}
%    \caption{ZenScore distribution for VTEI.}
%    \label{fig:benchmark_zenscore_vtei}
%\end{figure}

%Figure \ref{fig:average_across} shows a scatterplot comparing the average mAP across the formats for all the model categories versus the number of parameters of each backbone. It can be seen that full-MLPs, heterogeneous, and C2f architectures concentrate the models with the best mAPs at the lowest number of parameters. In this exact figure, a circle is used to highlight the baseline models, where it can be seen that although they are among the top performers
%, there is still room for improvement in the reduction of parameters, which can be identified in the graph by the region engulfed by the square, with all the models with an mAP over 0.50 and less than 1M parameters.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figurinhas/averageacross.png}
%    \caption{Average mAP across different formats versus the number of parameters}
%    \label{fig:average_across}
%\end{figure}

% \sout{\subsection{Search Algorithm Performance }}

\subsubsection{Impact of the Diversity Index}
\label{sec:res:search}

Based on the findings from Section \ref{sec:results:bench}, SHIST was approved as the reference event encoding for the Chimera-NAS algorithm. Furthermore, as shown in Figure \ref{fig:cor_data_format}a and Table \ref{tab:max_correlation}, the weights were set to $\mathbf{W} = [0.6, 0.4, 0.0]$, which correspond to weights of Zen-Score, MACs and NTK proxies. To assess the distribution of different blocks across architectures and to determine whether diversity contributes to performance enhancements, multiple searches were conducted by varying the parameter $\alpha$ from Equation \ref{eq:diversity_index} within the range of 0.05 to 1.0. These searches were conducted using Algorithm \ref{alghtm:chimera} with 50 individuals, 1,000 iterations, and a maximum parameter limit $MAX_{\text{Params}}$ of 10M per architecture. To evaluate the effectiveness of the searches, the top 5 architectures for each $\alpha$ value were trained for 100 epochs, and their final mAP for PEDRo was averaged. 
%The results are presented in Figure \ref{fig:map_search_10m}, which indicates that 
According to the results, the best mAP performance was achieved at $\alpha = 0.05$, surpassing the other configurations by approximately +2.0. More details are presented in the Supplementary Material.

%\subsubsection{Diversity Analysis}
%\label{sec:res:diversity_}




%It can be noticed that, depending on the value of $\alpha$, the search will tend towards the extremes. For low alpha values, the diversity tends toward 1, while for values higher than 0.4, it tends toward 1.0. Specifically, higher alpha values lead to full-WaveMLP architectures, as expected from Figure \ref{fig:zen-distribution}, which showed that this category of architectures tends to have a higher Zen Score. 

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figurinhas/average_mAP_10M.eps}
%     \caption{Average of the top-5 performers resulting from the Chimera-NAS search across different alpha values, at 10M parameters constraint, for the PEDRo dataset.}
%     \label{fig:map_search_10m}
% \end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{figurinhas/diversity_10m_2.eps}
%    \caption{Analysis of the average Diversity of the final population when running Chimera-NAS with a parameter constraint of 10M, a population of 50 individuals, and 1,000 iterations.}
%    \label{fig:diversity_10M}
%\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{figurinhas/zenScore_boxplot.png}
%    \caption{Distribution of the Zen Score according to different architectures.}
%    \label{fig:zen-distribution}
%\end{figure}

%\subsection{Chimera-NAS Runtime Analysis}
%\label{sec:results:runtime}


\subsection{Search Results}
\label{sec:results:search_archs}

%Considering the analysis conducted in the previous sections, 
To conduct the search of the architectures, the Algorithm \ref{alghtm:chimera} was repeated with the same population and iteration parameters, utilizing the $\textbf{W}$ obtained from Section \ref{sec:results:bench} and the $\mathbf{\alpha} = 0.05$ established in Section \ref{sec:res:search} for three constraints of $MAX_{\text{Params}}$ set to 3M, 5M, and 10M. Generally, after the search, the composition of the population regarding block types remained nearly identical across all individuals, with only minor variations in other parameters such as the number of channels, heads, and multipliers. Table \ref{tab:chimera_compostion} presents the blocks within the Chimera Layers obtained as a result of search for these three cases. After 1,000 iterations for each scenario, the population exhibited the same composition and arrangement of blocks, with differences confined to the number of channels and other parameters specific to the blocks.
\par 

To optimize the number of trainable parameters, Chimera-NAS recommends positioning the MaxViT block within the earlier layers of Chimera to enhance the capture of global data context. The C2f block is a convolutional component that accelerates processing and enhances model accuracy, primarily concentrating on local feature extraction. In contrast, the SSM module in the Mamba architecture is specifically designed to address both long- and short-term dependencies. Consequently, it can be inferred that the Chimera-3M model places a greater emphasis on spatio-temporal modeling compared to the Chimera-5M. Furthermore, the WaveMLP block in Chimera Layer 4 facilitates the encoding of both local and global features.

For the Chimera-10M model, the initial phase focuses on learning short- and long-term dependencies while engaging in local feature extraction. Global feature extraction occurs in Chimera Layers 3 and 4 through the WaveMLP and MaxViT blocks.




\begin{table}[]
\centering
\footnotesize
\caption{Composition of the Chimera Layer for architectures found with the Chimera-NAS algorithm under different parameters constraints.}
\label{tab:chimera_compostion}
\begin{tabular}{|c|c|c|c|}
\hline
% \begin{tabular}[c]{@{}c@{}}Chimera \\ Layer \end{tabular}    
\diagbox[width=11em]{Chimera Layer}{Params}& 3M      & 5M      & 10M     \\ \hline \hline
Chimera Layer 1& MaxViT  & MaxViT  & Mamba   \\ \hline
Chimera Layer 2 & Mamba   & C2f     & C2f     \\ \hline
Chimera Layer 3 & C2f     & Mamba   & WaveMLP \\ \hline
Chimera Layer 4 & WaveMLP & WaveMLP & MaxViT  \\ \hline
\end{tabular}
\end{table}

\subsection{Comparison with the state-of-the-art}
\label{sec:results:sota}






% Table \ref{tab:pedro} 
Figure \ref{fig:results} presents the architectures generated from the three searches—Chimera-3M, Chimera-5M, and Chimera-10M—alongside comparisons to other works in the literature for PEDRo. The results from ReYOLOv8 only include outcomes before the application of Random Polarity Suppression (RPS) \cite{reyolov8}, an augmentation technique specific to VTEI that has not yet been investigated alongside other formats, and therefore, were not applied to the Chimeras using SHIST. The MaxViT-Base model adheres to the backbone specifications from RVT \cite{rvt} but was trained under the same setup as the other models in this work.
\begin{figure}
    \centering
    \includegraphics[scale=0.25]{figurinhas/chimera_results.png}
    \caption{Comparison between the results and the state-of-the-art for the dataset PEDRo.}
    \label{fig:results}
\end{figure}

The Chimera networks demonstrate strong performance, particularly at lower scales. Specifically, Chimera-3M performs similarly to ReYOLOv8n but with 1.5 times fewer parameters. Meanwhile, Chimera-5M shows an improvement in mAP of approximately 9\% compared to a similarly scaled ReYOLOv8n, achieving a comparable mAP to ReYOLOv8s, but with a model size that is 1.7 times smaller. However, Chimera-10M does not yield significant improvements over Chimera-5M or other similarly scaled models in the literature. One potential explanation for this is that at the 10M parameter constraint, the search space becomes larger than at lower scales, which may complicate the search process.



%\textcolor{red}{YOU NEED MORE COMMENTS ON THE RESULTS. LIKE WHY THERE IS A JUMP FROM CHIMERA 3M TO 5M, BUT THERE IS NO MUCH IMPROVEMENT FROM 5M TO 10M?
%ALSO, YOU SHOULD NOT ADD SCALES HIGHER THAN WHAT YOU EXPLORED UNLESS YOU EXPLICITLY STATE THAT CHIMERA CAN ACHIEVE PERFORMANCE CLOSE TO HIGHER CAPACITY MODELS.
%LASTLY, I DO NOT THINK YOU SHOULD ADD RE-YOLO TO YOUR RESULTS.}

%\begin{table}[ht!]
%\centering
%\footnotesize
%\caption{Comparison between the results and the state-of-the-art for the dataset PEDRo.}
%\label{tab:pedro}
%\begin{tabular}{cccc}
%\hline
%\textbf{Model}                                                         & \textbf{Network}  & \textbf{Parameters} & \textbf{\begin{tabular}[c]{@{}c@{}}mAP\end{tabular}} \\ \hline
%\begin{tabular}[c]{@{}c@{}}Chimera-3M\\ (this work)\end{tabular}       & Hybrid + RNN      & 3.0M                & 59.5                                                             \\%
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8n\\ \cite{reyolov8}\end{tabular}     & CNN + RNN         & 4.7M                & 59.0                                                             \\
%\begin{tabular}[c]{@{}c@{}}Chimera-5M\\ (this work)\end{tabular}       & Hybrid + RNN      & 4.9M                & 64.2                                                             \\
%\begin{tabular}[c]{@{}c@{}}Chimera-10M\\ (this work)\end{tabular}      & Hybrid + RNN      & 7.2M                & 64.9                                                             \\
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8s\\ \cite{reyolov8}\end{tabular}     & CNN + RNN         & 8.4M                & 64.5                                                             \\
%\begin{tabular}[c]{@{}c@{}}MaxViT-Baseline\\ (Adapted from \cite{rvt})\end{tabular} & Transformer + RNN & 9.2M                & 52.6                                                             \\
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8m\\\cite{reyolov8}\end{tabular}     & CNN + RNN         & 18.1M               & 66.5                                                             \\
%\begin{tabular}[c]{@{}c@{}}YOLOv8x\\ \cite{yolov8}\end{tabular}       & CNN               & 68.2M               & 58.6                                                             \\ \hline
%\end{tabular}
%\end{table}




%\begin{table}[]
%\centering
%\small
%\caption{Comparison with other approaches in the literature for the GEN1 dataset.}
%\label{tab:literature_gen1}
%\begin{tabular}{cccc}
%\hline
%\textbf{Model}                                                                    & \textbf{Network}     & \textbf{Parameters}  & \textbf{mAP}             \\ \hline
%\begin{tabular}[c]{@{}c@{}}Chimera-3M\\ (this work)\end{tabular}                  & Hybrid + RNN         & 3.0M                 & \multicolumn{1}{l}{44.6} \\
%\begin{tabular}[c]{@{}c@{}}RVT-T \\ \cite{rvt}\end{tabular}          & Transformer + RNN    & 4.4M                 & 44.1                     \\
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8n \\ \cite{reyolov8}\end{tabular}  & CNN + RNN            & 4.7M                 & 46.3                     \\
%\begin{tabular}[c]{@{}c@{}}Chimera-5M\\ (this work)\end{tabular}                  & Hybrid + RNN         & 4.9M                 & \multicolumn{1}{l}{46.0} \\ \hline
%\begin{tabular}[c]{@{}c@{}}Chimera-10M\\ (this work)\end{tabular}                 & Hybrid + RNN         & 7.2M                 & 46.3                     \\
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8s\\ \cite{reyolov8}\end{tabular}   & CNN + RNN            & 8.4M                 & 48.3                     \\
%\begin{tabular}[c]{@{}c@{}}DTSDNet-S\\ \cite{dstdnet}\end{tabular}   & Dual Pathway CNN     & 9.1M                 & 43.9                     \\
%\begin{tabular}[c]{@{}c@{}}HMNet-B1\\ \cite{hmnet}\end{tabular}      & HMNet                & 9.4M                 & 45.5                     \\
%\begin{tabular}[c]{@{}c@{}}S5-ViT-S\\ \cite{event-ssm}\end{tabular}  & Transformer + SSM    & 9.7M        %         & 46.6                     \\
%\begin{tabular}[c]{@{}c@{}}RVT-S \\ \cite{rvt}\end{tabular}          & Transformer + RNN    & 9.9M        %         & 46.5                     \\
%\begin{tabular}[c]{@{}c@{}}HMNet-L1\\ \cite{hmnet}\end{tabular}      & HMNet                & 11.4M       %         & 47.0                     \\
%\begin{tabular}[c]{@{}c@{}}AED\\ \textbackslash{}citeaed\end{tabular}             & CNN                  %& 14.8M                & 45.4                     \\ \hline
%\begin{tabular}[c]{@{}c@{}}S4D-ViT-B\\ \textbackslash{}citeevent-ssm\end{tabular} & Transformer + SSM    %& 16.5M                & 46.2                     \\
%\begin{tabular}[c]{@{}c@{}}ReYOLOv8m\\ \textbackslash{}cite reyolo\end{tabular}   & CNN + RNN            %& 18.1M                & 49.4                     \\
%\begin{tabular}[c]{@{}c@{}}S5-ViT-B\\ \textbackslash{}citeevent-ssm\end{tabular}  & Transformer + SSM    %& 18.2M                & 47.7                     \\
%\begin{tabular}[c]{@{}c@{}}RVT-B\\ \textbackslash{}citervt\end{tabular}           & Transformer + RNN    %& 18.5M                & 47.2                     \\
%\begin{tabular}[c]{@{}c@{}}SAST-CB \\ \textbackslash{}citesast\end{tabular}       & Transformer + RNN    %& 18.9M                & 48.2                     \\
%\begin{tabular}[c]{@{}c@{}}GET\\ \textbackslash{}citeget\end{tabular}             & Transformer + RNN    %& 21.9M                & 47.9                     \\
%\begin{tabular}[c]{@{}c@{}}RED\\ \textbackslash{}citered\_megapixel\end{tabular}  & CNN + RNN            %& 24.1M                & 40.0                     \\
%\begin{tabular}[c]{@{}c@{}}DTSDNet-M \\ \textbackslash{}citedstdnet\end{tabular}  & Dual Pathway CNN     %& 25.7M                & 47.7                     \\
%\begin{tabular}[c]{@{}c@{}}HMNet-B3\\ \textbackslash{}citehmnet\end{tabular}      & HMNet                %& 29.8M                & 45.2                     \\
%\begin{tabular}[c]{@{}c@{}}HMNet-L3\\ \textbackslash{}citehmnet\end{tabular}      & HMNet                %& 33.2M                & 47.1                     \\ \hline
%\multicolumn{1}{l}{}                                                              & \multicolumn{1}{l}{} %& \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    
%\end{tabular}
%\end{table}


==> sec/5_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This work presents a two-stage NAS approach specifically aimed at Event-Based Object Detection. Instead of exploring variations of particular blocks, the architecture search centered on combining blocks from various paradigms within the literature to create more robust architectures. The resulting framework, named Chimera-NAS, utilizes proxies to assess architecture performance on test sets without requiring extensive training, enabling the examination of over 1,000 structures within a few hours. To manage the diversity of blocks within the architectures, a diversity index was introduced to quantify this aspect. The results obtained on the PEDRo dataset demonstrated significant improvements, achieving performance comparable to state-of-the-art models while maintaining an average parameter reduction of 1.6x.







\section{Future Works}
\label{sec:futureworks}

Future work will explore more blocks, alternative types of memory cells, such as State Space Models, and larger datasets, specifically Prophesee's GEN1 and 1MegaPixel.
